Efficiently Computing Nash Equilibria in Adversarial Team Markov Games

Computing Nash equilibrium policies is a central problem in multi-agent reinforcement learning that has received extensive attention both in theory and in practice. However, provable guarantees have been thus far either limited to fully competitive or cooperative scenarios or impose strong assumptions that are difficult to meet in most practical applications. In this work, we depart from those prior results by investigating infinite-horizon \emph{adversarial team Markov games}, a natural and well-motivated class of games in which a team of identically-interested players -- in the absence of any explicit coordination or communication -- is competing against an adversarial player. This setting allows for a unifying treatment of zero-sum Markov games and Markov potential games, and serves as a step to model more realistic strategic interactions that feature both competing and cooperative interests. Our main contribution is the first algorithm for computing stationary $\epsilon$-approximate Nash equilibria in adversarial team Markov games with computational complexity that is polynomial in all the natural parameters of the game, as well as $1/\epsilon$. The proposed algorithm is particularly natural and practical, and it is based on performing independent policy gradient steps for each player in the team, in tandem with best responses from the side of the adversary; in turn, the policy for the adversary is then obtained by solving a carefully constructed linear program. Our analysis leverages non-standard techniques to establish the KKT optimality conditions for a nonlinear program with nonconvex constraints, thereby leading to a natural interpretation of the induced Lagrange multipliers. Along the way, we significantly extend an important characterization of optimal policies in adversarial (normal-form) team games due to Von Stengel and Koller (GEB `97).

==> macros/nlp-env.tex <==
%%%% https://tex.stackexchange.com/questions/83918/labeled-linear-program-with-labeled-equations-and-wide-objective-function
\usepackage{xkeyval}
\makeatletter
\newlength{\LP@lh@boxwidth}      %% width of first box, set automatically within environment
\setlength{\LP@lh@boxwidth}{0pt}
\newlength{\LP@lh@boxsep}        %% distance between two boxes.  Default is `2em`.  Can be overridden by using key `boxsep=<length>`
\setlength{\LP@lh@boxsep}{2em}
\newcommand{\LP@lh@content}{}
\newcommand{\LP@lh@tagname}{}    %% set by user using key `tagname=<name of tag>`
\define@key[LP]{lhbox}{boxsep}[1em]{\setlength{\LP@lh@boxsep}{#1}}
\define@key[LP]{lhbox}{content}[]{\renewcommand{\LP@lh@content}{#1}}
\define@key[LP]{lhbox}{tagname}[]{\renewcommand{\LP@lh@tagname}{#1}}
\newenvironment{tagblock}[1][]%
                         {\setkeys[LP]{lhbox}{tagname,boxsep,#1}\relax%
                          \settowidth{\LP@lh@boxwidth}{\tagform@\LP@lh@tagname}%
                          \noindent%
                          \parbox{\LP@lh@boxwidth}{\begin{align}\tag{\LP@lh@tagname}\LP@lh@content\end{align}}%
                          \hspace*{\LP@lh@boxsep}%
                          \begin{minipage}{\linewidth-\LP@lh@boxwidth-\LP@lh@boxsep}}%
                         {~\end{minipage}}
\makeatother

% \makeatletter
% \newlength{\LP@lh@boxwidth}      %% width of first box, set automatically within environment
% \setlength{\LP@lh@boxwidth}{0pt}
% \newlength{\LP@lh@boxsep}        %% distance between two boxes.  Default is `2em`.  Can be overridden by using key `boxsep=<length>`
% \setlength{\LP@lh@boxsep}{2em}
% \newcommand{\LP@lh@content}{}
% \newcommand{\LP@lh@tagname}{}    %% set by user using key `tagname=<name of tag>`
% \define@key[LP]{lhbox}{boxsep}[1em]{\setlength{\LP@lh@boxsep}{#1}}
% \define@key[LP]{lhbox}{content}[]{\renewcommand{\LP@lh@content}{#1}}
% \define@key[LP]{lhbox}{tagname}[]{\renewcommand{\LP@lh@tagname}{#1}}
% \newenvironment{tagblock2}[2][]%
%                          {\setkeys[LP]{lhbox}{tagname,#2,#1}\relax%
%                           \settowidth{\LP@lh@boxwidth}{\tagform@\LP@lh@tagname}%
%                           \noindent%
%                           \parbox{\LP@lh@boxwidth}{\begin{align}\tag{\LP@lh@tagname}\LP@lh@content\end{align}}%
%                           \hspace*{\LP@lh@boxsep}%
%                           \begin{minipage}{\linewidth-\LP@lh@boxwidth-\LP@lh@boxsep}}%
%                          {~\end{minipage}}
% \makeatother

==> sections/experiments.tex <==
\section{Experimental Setup}

In this section we lay down all the implementation details of the multi-agent environment created as well as the experiments conducted to support our theoretical findings.

\begin{figure}[!htb]
  \begin{minipage}{0.48\textwidth}
     \centering
     \includegraphics[width=120pt]{figures/movement.png}
     \caption{Action space of each agent}\label{Fig:action_space}
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
     \centering
     \includegraphics[width=120pt]{figures/AdvTeamGames.png}
     \caption{Environment sketch.}\label{Fig:Data2}
  \end{minipage}
\end{figure}

\paragraph{States/Actions/Rewards} Consider an $n \times n$ grid-world environment with $N = 2$ agents and an adversary, each placed randomly on the grid following a uniform distribution over the coordinates. In the environment, there are also 2 landmarks in fixed locations. Each positional configuration of the agents on the grid maps to a distinct state in the MDP. Figure 2 shows a configuration of the agents in the grid as well as the 2 landmarks at the 2 opposite corners of the grid. Each agent has 4 actions mapping to all cardinal directions. The agents take actions simultaneously and transitions happen synchronously. A reward signal of $+1$ is distributed to the team if every member covers a landmark. If this happens before the adversary reaches a landmark, the adversary is rewarded with $-1$. However, if adversary reaches any landmark before all members of the team complete their objective, it receives a reward of $+1$ and the team experiences a reward of $-1$. 

\paragraph{Nash Equilibria} To show convergence, we plot the Frobenius norm of consecutive joint policies, the average estimated value of the team and also provide some screenshots of agents in a multi-grid environment demonstrating behavior.
\begin{figure}[!htb]
  \begin{minipage}{0.48\textwidth}
     \centering
     \includegraphics[width=210pt]{figures/policies.png}
  \end{minipage}\hfill
  \begin{minipage}{0.48\textwidth}
     \centering
     \includegraphics[width=210pt]{figures/value.png}
     %\caption{Interpolation for Data 2}\label{Fig:Data2}
  \end{minipage}
  \caption{On the left we plot the Frobenius norm of the joint policies and on the right, the estimated value of the team at each time-step.}\label{Fig:plots}
\end{figure}

Below we also provide interesting screenshots we collected at the end of training:

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\textwidth]{figures/3x3_results/trajectory.png}
    \caption{A sample trajectory when all players are in Nash equilibrium.}
    \label{fig:my_label}
\end{figure}

Observe how the agents in 
